Subset Node Anomaly Tracking over Large Dynamic Graphs

Tracking a targeted subset of nodes in an evolving graph is important for many real-world applications. Existing methods typically focus on identifying anomalous edges or finding anomaly graph snapshots in a stream way. However, edge-oriented methods cannot quantify how individual nodes change over time while others need to maintain representations of the whole graph all time, thus computationally inefficient. This paper proposes \textsc{DynAnom}, an efficient framework to quantify the changes and localize per-node anomalies over large dynamic weighted-graphs. Thanks to recent advances in dynamic representation learning based on Personalized PageRank, \textsc{DynAnom} is 1) \textit{efficient}: the time complexity is linear to the number of edge events and independent on node size of the input graph; 2) \textit{effective}: \textsc{DynAnom} can successfully track topological changes reflecting real-world anomaly; 3) \textit{flexible}: different type of anomaly score functions can be defined for various applications. Experiments demonstrate these properties on both benchmark graph datasets and a new large real-world dynamic graph. Specifically, an instantiation method based on \textsc{DynAnom} achieves the accuracy of 0.5425 compared with 0.2790, the best baseline, on the task of node-level anomaly localization while running 2.3 times faster than the baseline. We present a real-world case study and further demonstrate the usability of \textsc{DynAnom} for anomaly discovery over large-scale graphs.

==> acmart-1.80/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-1.80/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> cut-offs.tex <==
% general node/graph  monitoring

%(e.g., keeping track of suspicious nodes in a large social network, watching nodes of specific types in a massive heterogeneous graph)[\textcolor{red}{BJ: Examples could be put into intro.}].
% New problem: subset node monitoring 

% an instance of the application
% \footnote{For example, when analyze how \textit{Donald Trump} changes in Wikipedia hyperlink graph (about 6.4M nodes in total) over time, we are only interested in a subset of node $S = \{"\text{Donald-Trump}"\}$ and $|S|$ =1. We may want to avoid the computation of the other non-targeted nodes (places, food, events, ...) for efficiency purpose.}

% propose the problem

However, most of the computational time is used for small values as the iteration continues. In practice, those small values are less important than the large values (e.g., Top-k PPR values), thus neglected.



% To obtain dynamic embedding vectors, the general idea is to obtaindynamic PPVs and then project these PPVs into embedding spaceby using two kernel functions [30,42]. In this section, we presentour proposed methodDynamicPPEwhere it contains two maincomponents: 1) an adaptive precision strategy to control the esti-mation error of PPVs. We then prove that the time complexity ofthis dynamic strategy is still independent on��. With this qualityguarantee, learned PPVs will be used as proximity vectors and be"projected" into lower dimensional space based on ideas ofVerse[39] andInstantEmbedding[30]. We first show how can we get highquality PPVs and then present how use PPVs to obtain dynamicembeddings. Finally, we give the complexity analysis.

% \red{The proposed method should (or maybe) split into 3 parts. The first part is theoretical foundations of dynamic anomaly detection based on PPVs. Maybe give a chance to unify previous works. The second section is to analyze and present our proposed method. The third section is to analyze the theoretical guarantees w.r.t anomaly scores and qualities and also the run time complexity analysis. This part should finish as we argue the efficiency compared with previous methods.}


% \red{XZ: add a table talking about time complexity, and could the method handle individual anomaly tracking }
% \subsection{DynamicPPE} 
% \textcolor{red}{should we put it in method or related work} 

%\subsection{DynamicPPE with Weighted Push} Extend DynamicPPE with weighted adjacent matrix, and incremental push (with adjusted transition weights). We prove the incrementally PPR in Appendix \ref{appendix:unweighted-ppr-update}.

% \footnote{\url{https://www.aberdeennews.com/story/opinion/columns/2021/10/11/al-franken-makes-comeback-include-run-office/6053193001/}}

% Arnold Schwarzenegger:
% \begin{itemize}
%     \item In 2003, Arnold Schwarzenegger won the California gubernatorial election as his first politician role.
%     \item In 2008, Arnold began campaigning with McCain as the key endorsement for McCain's presidential campaign.  
%     \item In 2010, mid-term election.
%     \item After 2011, Arnold reached his term limit as Governor and returned to acting.
% % \end{itemize}

% Al Franken:
% \begin{itemize}
%     \item In 2002, Al Franken consider his first race for office due to the tragedy of Minnesota Sen. Paul Wellstone.\footnote{\url{https://www.aberdeennews.com/story/opinion/columns/2021/10/11/al-franken-makes-comeback-include-run-office/6053193001/}}
%     \item In 2004, The Al Franken Show aired.
%     \item In 2007, Al Franken announced for candidacy for Senate.
%     \item In 2008, Al Franken won election.
%     \item In 2012, Al Franken won re-election.
%     \item In 2018, Al Franken resigned.
% \end{itemize}

\clearpage


\xingzhiswallow{
\subsection{Issue with edge anomaly detection}
The edge anomaly detection algorithm assign anomaly score to each edge, however, it can not measure the node-level anomaly since if there is only a few edge associated with a node across snapshot, the node does not change in the snapshot without edges involving this node, regardless of its neighbors' evolution.
}

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.

% \begin{acks}
% %add fundings

% \end{acks}

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.


% \red{we use max changes happen in top degree nodes $\pi_{\alpha}$ as grpah-level anomaly score}
% \paragraph{All-Tracking} Tracks all nodes once the node emerged in the graph.
% \paragraph{Top Node Tracking}: Incrementally add top-degree nodes into the tracking list from each snapshots. 

% \paragraph{Def-Tracking} Track the pre-defined nodes in the graph.

% \begin{algorithm}[ht]
% \caption{$\textsc{DynAnom}_{graph}(p_s^0, ... ,P_s^T)$}
% \begin{algorithmic}[1]
% \State $\delta_{\mathcal{G}} = \bm 0 \in \mathbb{R}^T$

% \State \textbf{return} $\bm W_s^t = [\bm w_s^1,\bm w_s^2,\ldots, \bm w_s^T], \forall s\in S$. 
% \end{algorithmic}
% \label{algo:dynanom-node}
% \end{algorithm}

% \paragraph{Active-Tracking} Tracks all nodes, but selectively update PPV based on the significant edge update, in terms of degree and $\Delta_{\{ p_s,r_s \}}$ changes.

%Focus on nodes, tracking the changes of a node across different snapshots and calculate the PPV changes.



% Given the node heterogeneity and size in the real-world graphs (), we may only interested 
% Such anomalies may constantly happen across different parts of graph, given that the real-world graphs are large-scale and fast-growing.  

% those methods may fail to monitor a subset nodes of interest (e.g., suspicious grey-list nodes). 

% but fail to further localize the specific anomalies nodes, or efficiently quantify the anomaly score of individually interesting nodes due to expensive re-training or fine-tuning.

% Additionally, given that the anomalies are constantly occurring, a global anomaly detector may always signify as positive, and becomes pointless unless it could localize where the anomalies actually happen. 
% Meanwhile, the scale and dynamics of graph also requires high efficiency. Thus, the following two important problems still remain unsolved : 
% 1). How to localize anomalous nodes in dynamic graphs?  
% 2). How to efficiently quantify the anomaly scores of individual nodes as the graph evolves? 

% In this paper, we propose a scalable and efficient PageRank-based anomaly detection algorithms over dynamic graphs. 
% In this paper, we propose an unifying algorithm to solve both aforementioned problems, which can effectively localize anomalies at the finest node level, and be capable of efficiently processing large dynamic graphs in an incremental fashion. 




% \textbf{1:} Coarse anomalous node candidates selection based on heuristics (e.g., the most active nodes in each time period). 
% \textbf{2:} Finer anomalous node selection based on the score derived from the highly efficient dynamic node embedding of time complexity ($\frac{\Delta m}{\epsilon \alpha}$), regardless of graph node size.   




%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.


% BJ: (e.g., grey-listed nodes), searched Google scholar, only one paper used this term.
% Monitoring a targeted subset of nodes (e.g., grey-listed nodes) in an evolving graph is critical for many real-world applications.



% We argue that the node-level anomaly could also capture the global anomaly given the fact that global anomaly could be decomposed to many node-level anomalies. Additionally, to describe the node in a graph, a well-known measure is Single-Source Personalized PageRank (SS-PPR). Following the recent advances in efficient local algorithms for SS-PPR in dynamic setting, we integrate SS-PPR for anomaly detection, and introduce in Section \ref{sec:ppr}.

% We believe that the graph-level anomaly consists of node and edge anomalies, reflecting the global properties, thus could be represented by finer-level anomalies.  
% In contrast, edge-level anomaly measures the fitness of two local nodes it connected with, but makes the scope too narrow and unavailable to the nodes without direct link. In other words, it may ignore the local community information when deciding if the edge-level anomaly occurs. 
% Node level as the intermediate, consisting the node-level community properties and fine-level local structure, could better capture the anomaly for both macro and micro anomalies. 



% In this paper, we restrict out attention on node-level anomaly detection and extend the node anomaly to graph anomaly.
%Therefore, focusing more on local perturbations, personalized PageRank is favored on the anomaly node identification.


\xingzhiswallow{
\sout{\red{Instead,} Node representation-based methods are the most satisfying approaches, but most of them \cite{perozzi2014deepwalk,grover2016node2vec,yu2018netwalk} may computationally suffer from large node size, \red{e.g., the size of our motivating example}, and waste computations on the nodes falling out of the target subset. In our example where we have million-scale graph over thousands of snapshots, those methods may fail to finish.}
}

 %, causing extra overhead for re-alignment (e.g., $\mathcal{O}(n^3 T) $ for Procrustes analysis \cite{gower1975generalized, wang2008manifold}, $T$ is the number of snapshots and $n$ is the number of nodes). 

%\cite{tsitsulin2021frede}
% recent local methods could save 
% but anomaly for local methods was not explored.
% our paper extend local method to weighted graph and explore the anomaly 

% \item \textcolor{red}{Copied from abstract: Our three major contributions are:
% \textit{ \textbf{1.}} A more applicable efficient local node representation based on incremental PPVs over evolving graphs, whose per-node time complexity is bounded by edge events ($\Delta m$) and error parameter($\epsilon$) regardless of graph node size.  \textit{ \textbf{2.}} An unified framework for both node-level anomaly localization and global snapshot-level anomaly detection with theoretical guarantees.
% \textit{ \textbf{3.}} Analysis on two new, large, real-world dynamic graphs of people and countries across 30 years. With the scarcity of annotated-\textit{anomaly} graphs, these resources provide fresh opportunities for human-interpretable anomaly detection in graph mining community.}


%2. The are all sudden changes from original patterns, either in global or local resolution, and we define the anomaly as the sudden changes in feature space.\\

% 3.1 How to construct features?  PageRank as global graph-level features. Node embeddings as local node-level features.  \\

% 3.2 How to efficiently construct features for evolving graphs?  \\

% 3.2.1. Embedding Space consistency\\

% 3.2.2. Algorithm Efficiency \\

% 4. How to define anomaly over feature space? \\

% 4.1 $l_1$ distance, \\

% 4.2 Derivatives of changes.\\

% 4.3 Difference in clustering.\\



% Many real-world networks (e.g., online transaction, social network interaction) are large-scale and evolving at a fast pace, involving nodes and edges being added or deleted.
%Monitoring anomalies over a fast-growing graph is critical to detect online transaction fraud, social spam, malware, etc. 

% static graph
%In a static graph consisting of a fix number of vertices and edges, graph-level anomaly considers the global properties of graph, and measure the deviation of the selected properties against the \textit{norm}, which are observed from the other instances in the same graph-family. For example, the power-law node degree distribution, betweenness, etc.

% \citet{beutel2013copycatch} 
%We notices that many PageRank-based methods \cite{yoon2019fast} were developed. 


%It neither has ability to track changes of suspicious nodes, nor to determine which edges are unwelcome.  
% In practice, the local subtle anomalies may constantly occur (e.g., online frauds are always going on in a large transaction network), spotting local anomalies is critically useful to inspect and understand the problem, instead of flagging the whole snapshot as anomaly.  
% From theoretical perspective, \citet{lee2003perturbation} suggests that the global PageRank is rather stable w.r.t. the edge perturbation, so the global PageRank may not be sensitive to the local malicious changes, resulting in many false negative.
%\todo{We may need to highlight local (subtle) changes are important if our assumption is true.}

%Many streaming based methods \cite{chang2021f,eswaran2018sedanspot} were proposed. 
%Many edge streaming anomaly detection algorithms \cite{bhatia2020midas, eswaran2018spotlight} were proposed.


%thus unable to monitor the node status change resulted from the community evolution as the Trump-Melania example shows.

% Similarly, edge-level anomaly detection identifies the unexpected edges. The fitness of an existing edge could be determined by the node properties (either node embeddings or hand-crafted features) of the nodes on the edge's endpoints. 

% node anomaly 
% Node-level anomaly detection is equivalent to identify the outliers w.r.t. node properties, that is - the nodes belonging to neither community or those of unexpected high degrees \textcolor{red}{CITE}. The definition of anomaly is hueristic and application-dependant, the most recent works use powerful network embeddings as the node representation for outlier detection. 


%Compare to the global anomaly, local changes are more subtle, thus it might not be significant enough to affect global graph property.


%For example, we may want to quantify the anomaly of a single persons in a million-scale dynamic graph. A straightforward pruning of irrelevant nodes from the graph may remove useful network structure information and dramatically change the graph topology. 
%And calculating all node embeddings across times then extract the node subset may less computationally-budgeted, even becomes impractical if the graph size is large (millions of nodes) and time horizon is long (thousands of snapshots). Therefore, an efficient subset node representation over large dynamic graph is critical.


% \red{not scalable} 
%However, since there is no embedding space alignment across time, the outliers can be only identified within each snapshot, which is more like a static node anomaly detection. Moreover, This method is inapplicable to large graph with upcoming new nodes because the used AutoEncoder  is not scalable and expandable. % \red{not scalable} 

%Likewise, JODIE \cite{kumar2019predicting} leverages Recurrent Neural Networks (RNNs) to model the node embedding trajectories changes as the graph evolves. 
%This model aims to predict the future node embeddings based on the previous interaction history, and model the node state based on the learnt latent representation.

% shortcomings of above methods
% However, considering the large-scale and fast-grow property of real-world graph, efficiently updating node representation becomes the bottleneck. 
% Moreover, in order to compare the node representation across different time, it needs a consistent embedding space alignment, which imposes extra overhead when calculating the node-level anomaly score. 
% Most importantly, the above methods are not good fit for the task of \textit{Local node-level anomaly by queried nodes} where we only care about a subset nodes of interest, as described in Definition \ref{def:node-track-def}. 
% For example, we may want to quantify the anomaly of persons in a heterogeneous graph containing the interactions both people, events, locations, etc. 
% A straightforward pruning of irrelevant nodes from the graph may remove useful network structure information and dramatically change the graph topology. 
% And calculating all node embeddings across times then extract the node subset may less computationally-budgeted, even becomes impractical if the graph size is large (millions of nodes) and time horizon is long (thousands of snapshots). Therefore, an efficient subset node representation over large dynamic graph is critical.

%Single-Source Personalized PageRank (SS-PPR) \cite{page1999pagerank}, could be leveraged for node representation. 
%for Single-Source Personalized PageRank (SS-PPR)

% We generalize the PPV approximation for incorporating node interaction frequency, which will be detailed in Section \ref{sec:notation-prelim} and Section \ref{sec:ppr}. We summarize the properties of algorithms in Table \ref{tab:algo-comparison}.






% \begin{table}[ht]
% \caption{The comparison of supported features between DynAnom and other methods.}
% \centering
% \begin{tabular}{p{0.15\textwidth}|rrrr|r}
% \toprule
%   \diaghead{\hskip 25mm }%
% {Feature}{Method} & \rotatebox[origin=c]{75}{SedanSpot\cite{eswaran2018sedanspot}} & \rotatebox[origin=c]{75}{AnomRank\cite{yoon2019fast}} & \rotatebox[origin=c]{75}{NetWalk\cite{yu2018netwalk}}  & \rotatebox[origin=c]{75}{DynPPE\cite{xingzhi2021subset}}  & \rotatebox[origin=c]{75}{\textbf{DynAnom}}  \\
% \midrule 
% Node-level Rep. &  \redxmark &  \redxmark & \bluecheck  & \bluecheck  & \bluecheck  \\
% Node Tracking &  \redxmark &  \redxmark &  \redxmark &  \bluecheck &  \bluecheck \\
% Multi-Edge & \bluecheck &  \bluecheck&  \bluecheck &  \redxmark&  \bluecheck\\
% Edge Add/Delete & \redxmark  & \bluecheck & \redxmark & \bluecheck &  \bluecheck \\
% Edge-stream & \bluecheck & \bluecheck & \redxmark  &  \bluecheck&  \bluecheck\\
% Score function-based & \bluecheck & \bluecheck & \bluecheck  &  \redxmark &  \bluecheck\\
% \bottomrule
% \end{tabular}
% \label{tab:algo-comparison}
% \end{table}

\xingzhiswallow{
\subsubsection{Selective Lazy Push}
Since our goal is to signify the changes in node status by comparing the PPVs before and after edge events, we may want to skip the edges causing minor PPV changes until it accumulates to invoke the push subroutine.

\red{[BJ: The following theorem should be move to preliminary part. Or we can present here as a generalized version.]}

\begin{theorem} \cite{lee2003perturbation} The bounds on difference between the old PPR vector  $\pi^{t-1}$ and new PPR vector $\pi^t $ is :
\begin{equation}
    || \pi_s^{t-1} -  \pi_s^t  ||_1 \leq \frac{2(1-\alpha)}{\alpha} \sum_ {i \in U} \pi_s^{t-1}(i), 
\end{equation}
 $U$ is the set of the updated nodes. The proof is in \cite{lee2003perturbation}.
 \label{theorem:alpha-bound-ppr}
\end{theorem}

From theorem \ref{theorem:alpha-bound-ppr}, we observe that a larger $\alpha$ (more chance to restart/teleport from/to the source node) would make smaller changes in PPR. 
If a node $v_i$ with large $\pi^{t-1}_i$ involved in edge changes, then, the upper bound also increases, leading to significant difference in the updated $\pi^{t}$.
It gives us a clue of when to actually need update PPR. In order to save time, we derived a selective lazy push procedure.

}

The most commonly used method is \textit{Power Iteration} \cite{page1999pagerank}, which approximates $\bm \pi_{s}$ iteratively:
\begin{align}
\bm \pi_{s}^{(t)} &= (1-\alpha)  \bm P^\top \bm \pi_{s}^{(t-1)} + \alpha \bm 1_s \textbf{ // Power Iteration}  \allowdisplaybreaks \nonumber\\
% &= (1-\alpha)^{t}  (\bm P^\top)^{t} \bm \pi_{s}^{(0)} + \alpha \sum_{i = 0}^{t-1}(1-\alpha)^{i} (\bm P^\top)^{i}\bm 1_s \nonumber  \allowdisplaybreaks\\
&= \alpha \bm 1_s \sum_{i = 0}^{t-1}(1-\alpha)^{i} (\bm P^\top)^{i} \text{ // assuming that }  \bm \pi_{s}^{(0)} = \bm 0.  \allowdisplaybreaks \label{eq:ppr-2} 
\end{align}


% The root reason of OOM is that the parameter size of NetWalk's AutoEncoder is related to $|\mathcal{V}|$ due to the 

% . Specifically, due to the reconstruction loss function in AE, the length of input/output one-hot vector is $|\mathcal{V}|$, making it computationally prohibitive when dealing with massive graph of large node set.  



% \textbf{DynPPE}, considering to be the unweighted version of \textbf{DynAnom} is always worse than its weighted counterpart. 





% \red{overall time complexity analysis here}


% \subsection{Node Vector Dynamically Maintenance} Instead of using the most up-to-date PPV for every update, we can maintain a temporal vectors with partially dimensions being updated every time.





%\subsection{Score functions ?}

% \subsection{Overall Proposed algorithm}
% \red{In the specific presentation style, union all these algorithms into one algorithm so that the proposed method looks novel and beauty.}

%We introduce the dataset, baseline methods, and experiment settings as following.


\xingzhiswallow{
\paragraph{Country Knowledge Graph (COUNTRY)}: We construct this country-level interaction graph from GDelta Project\cite{leetaru2013gdelt} \footnote{GDelta Homepage: \url{https://www.gdeltproject.org/}}. Each node is a country entity.
Each edge represent a inter-country \textit{conflict} interaction with Goldstein score \cite{goldstein1992conflict} smaller than -7.0\footnote{ Goldstein score ranges from -10.0 to 8.3,  measuring the intensity of conflict(negative) or cooperation(positive) inherent in different types of international events: e.g., -10.0: Military attack; -7.0: Threat with force specified; -3.0: Give warning, etc.}. Similarly, we study when did the countries shift foreign conflict focus as the global tension develop.  

}

%and use cluster-based measure to detect node-level anomaly. 
%However, in the original paper, the definition of anomaly is the edges that are not in the graph, making the task more similar to link prediction instead of anomaly detection.



%Its core PPV calculation module is equivalent to our proposed 

% \textcolor{red}{NetWalk does not finish in 10 hours.}


% \paragraph{F-Fade\cite{chang2021f}} factorizes the frequency of nodes-wise interactions in a edge stream, and use the likelihood of the observed interaction frequency as the anomaly score.

%shows one application using our proposed algorithm \textsc{DynAnom} over the Person-EventKG (3.1 million nodes and 6.7 million edges).

Note that the complexity is independent of the total node size. 

% \item Two large-scale real-world graphs for node level tracking: Person-EventKG and Country-EventKG are constructed as more human-interpretable resources for graph anomaly detection community. It brings more research opportunities for both algorithm benchmarking and data science discovery.  


\xingzhiswallow{
\subsection{Proof of PPV maintenance}
\label{sec:appendix-ppv-adjust-proof}
\begin{proof}
This proof follows the paradigm used in \cite{zhang2016approximate}. We start from the invariant property in Lemma \ref{lemma:ppr-invar}:
\begin{align}
p_s(i) + \alpha r_s(i) = (1-\alpha)\sum_{x \in N^{in}(i)}  \frac{ w_{(x,i)} p_s(x)}{d(x)} + \alpha \times 1_{t=s}, \forall i \in \mathcal{V}  
\end{align}

% Initially, this invariant holds and keeps $ \frac{r_s(i)}{d(i)} \leq \epsilon$ after applying Algo.\ref{algo:forward-local-push-weighted}. 
% When the new edge $(u,v,\Delta w_{(u,v)})$ arrives, it changes the out-degree of $u$, breaking up the balance for all invariant involving $d(u)$. Our goal is to recover such invariant by adjusting small amount of $p_s, r_s$. While such adjustments may compromise the quality of PPVs, we could incrementally invoke Algo.\ref{algo:forward-local-push-weighted} to update $p_s$ and $r_s$ for better accuracy afterwards. We denote the initial vectors as $p_s, r_s, d$ and post-change vectors as $p'_s, r'_s, d'$. 
When the new edge $(u,v,\Delta w_{(u,v)})$ arrives, we denote the initial vectors as $p_s, r_s, d$ and post-change vectors as $p'_s, r'_s, d'$. 

\paragraph{Update $p_s(u)$:}
% First, since $d'(u)$ is involved in $\frac{p_s(u)}{d'(u)}$, we should find an updated $p'_s(u)$ so that  $\frac{p_s(u)}{d(u)} = \frac{p'_s(u)}{d'(u)}$, which makes the invariants still hold for any $p_s(i)$ containing $\frac{p_s(u)}{d}$ in Eq.\ref{eq:u-invaraint-body}:
\begin{align}
    \frac{p'_s(u)}{d'(u)} &= \frac{p_s(u)}{d(u)}, \nonumber\\
    %p'_s(u) &= d'(u) \frac{p_s(u)}{d(u)},\nonumber\\
    p'_s(u) &= (d(u)+\Delta w_{(u,v)}) \frac{p_s(u)}{d(u)},\nonumber\\
            &= p_s(u) \frac{d(u)+\Delta w_{(u,v)}}{d(u)}, 
\end{align}

% Eq. \ref{eq:p-update-weighted-body-2} implies that we should scale up $p_s(u)$ to recover balance. This strategy is the general case of \citet{zhang2016approximate} for unweighted graphs where $\Delta w_{(u,v)} = 1$.

\paragraph{Update $r_s(u)$:} However, once we assign $p'_s(u)$, it breaks the invariant for $u$ since $p_s(u)+\alpha r_s(u) \neq p'_s(u)+\alpha r_s(u)$. Likewise, we maintain this equality by introducing $r'_s(u)$:
\begin{align}
    p_s(u) + \alpha r_s(u) & = p_s'(u) + \alpha r_s'(u) \nonumber\\
    % &= \sum_{x \in N^{in}(u)}  \frac{p_s(x)}{d(x)}, \text{  from eq. \ref{eq:u-invaraint-body}} \\
    &\text{Substitute $p'_s(u)$ from eq.\ref{eq:p-update-weighted-body}} \nonumber \allowdisplaybreaks\\
    % & = p_s(u)\frac{d(u)+\Delta w_{(u,v)}}{d(u)} + \alpha r_s'(u) ,\nonumber\\
    & = p_s(u) + \frac{\Delta w_{(u,v)} p_s(u)}{d(u)} + \alpha r_s'(u) , \nonumber \allowdisplaybreaks \\
    \Longrightarrow \alpha r_s'(u) - \alpha r_s(u) &= -\frac{\Delta w_{(u,v)} p_s(u)}{d(u)},\nonumber \allowdisplaybreaks\\
    % \alpha r_s'(u)  &= \alpha r_s(u) -\frac{\Delta w_{(u,v)} p_s(u)}{d(u)},\nonumber\\
    r_s'(u) &=  r_s(u) -\frac{\Delta w_{(u,v)} p_s(u)}{\alpha d(u)} 
\end{align}

% Eq. \ref{eq:r-update-weighted-body-2} implies that we should decrease $r_s(u)$. From a heuristic perspective, it's consistent to the behavior of BCA-algorithm which keeps taking mass from $r_s$ to $p_s$. In this updating case, we artificially create mass for $p'_s$ at the expense of $r_s$'s decrements. When $\Delta w_{(u,v)} = 1$ in case of unweighted graphs, this update rule is also equivalent to \citet{zhang2016approximate}.

% So far, we have the updated $p'_s(u)$ and $r'_s(u)$ so that all nodes (without direct edge update, except for $v$) keep the invariant hold. However, due to the introduction of $\Delta w_{(u,v)}$, the shares of mass pushed to $v$ is changes, breaking the invariant for $v$ as shown below:
% \paragraph{Update $r_s(v)$}
% \begin{align}
%     p_s(v) + \alpha r_s(v) & \neq (1-\alpha) \Bigl( \frac{ (w_{(u,v)} + \Delta w_{(u,v)})  p'_s(u)}{d'(u)} \Bigr. \nonumber\\
%     & \Bigl. + \sum_{x \in N^{in}(v) \setminus \{ u \} }  \frac{w_{(u,x)} p_s(x)}{d(x)} \Bigr) +\alpha \times \mathbbm{1}_{t=s} \nonumber
% \end{align}

% In order to recover the balance with minimal effort, we should update $r_s(v)$ instead of $p_s(v)$. The main reason is that any change in $p_s(v)$ will break the balance for $v$'s neighbors, similar to the breaks incurred by the change of $p_s(u)$. 
\paragraph{Update $r_s(v)$:} We present the updated $r'_s(v) = r_s(v)+\Delta $:
\begin{align}
p_s(v) + \alpha \Bigl(r_s(v)+\Delta \Bigr) &= (1-\alpha) \Bigl( \frac{\Delta w_{(u,v)} p'_s(u)}{d'(u)} + \Bigr. \nonumber\\
&\Bigl. \sum_{x \in N^{in}(v) }  \frac{w_{(u,x)} p_s(x)}{d(x)} \Bigr) +\alpha \times 1_{t=s}   \\
\text{Note that } \frac{p'_s(u)}{d'(u)} &= \frac{p_s(u)}{d(u)}, \text{ and}  \nonumber \\
p_s(v) + \alpha r_s(v) &= (1-\alpha)\sum_{x \in N^{in}(v)}  \frac{ w_{(x,v)} p_s(x)}{d(x)} \nonumber  \allowdisplaybreaks \\
&\hspace{-25mm}\text{Reorganize Eq. \ref{eq:invar-v-body} and cancel out $p_s(v), r_s(v)$, we have: } \nonumber \allowdisplaybreaks\\
\Longrightarrow \alpha \Delta &= (1-\alpha) \frac{ \Delta_{w_{(u,v)}} p'_s(u)}{d'(u)} \nonumber \allowdisplaybreaks\\
\Delta &= \frac{(1-\alpha)}{\alpha} \frac{ \Delta_{w_{(u,v)}} p_s(u)}{d(u)} \nonumber \allowdisplaybreaks\\
\text{Recall that } r_s'(v) &=  r_s(v) + \Delta \nonumber\\
&= r_s(v) + \frac{(1-\alpha)}{\alpha} \frac{\Delta_{w_{(u,v)}}p_s(u)}{d(u)}
\end{align}
We conclude the proof of Theorem \ref{theorem:dyn-adjust-weighted-graph}.

\end{proof}

}


\xingzhiswallow{
\begin{table}[h!]
    \centering
    \tiny
\begin{tabular}{p{0.1\linewidth} p{0.77\linewidth}}
\toprule
 Marker & Major Conflict Event \\
\midrule 
 \multicolumn{2}{c}{CHN (China)} \\
\midrule 
 CHN-1993 & Criticized the establishment of British Trade and Cultural Office in Taipei City. \\
 CHN-1999 & Belgrade Embassy Bombing: Chinese demonstrators protest throughout the country, attacking official U.S. property \\
 CHN-2008 & China-France over Tibetan sovereignty debate. Sudan violence against Chinese workers \\
 CHN-2009 & China-Australian over Tibetan sovereignty debate \\
 CHN-2010 & China-Japan Senkaku/Diaoyu Island Disputes \\
 CHN-2011 & China-Philippines-Vietnam South China Sea Territorial Disputes \\
 CHN-2014 & Severe Violence against Chinese in Vietnam over South China Sea  Disputes \\
 CHN-2016 & Taiwan-Strait tension. China-Philippines South China Sea Arbitration  \\
\midrule 
 \multicolumn{2}{c}{USA (U.S.)} \\
\midrule 
 USA-1994 & Battle of Mogadishu in Somalia (Black Hawk Down) \\
 USA-1998 & Operation Desert Fox in Iraq \\
 USA-1999 & Kosovo War \\
 USA-2001 & War in Afghanistan since 9-11  \\
 USA-2003 & Iraq War \\
 USA-2006 & Iraq (civil) War intensified \\
 USA-2008 & Pakistan–U.S. skirmishes \\
 USA-2011 & Military intervention in Libya \\
 USA-2016 & Syria Civil War (ISIS)  \\
 \bottomrule
\end{tabular}
    \caption{The global conflict events in China and the U.S.}
    \label{tab:country-events}
\end{table}
}


\xingzhiswallow{
\subsection{Static PPR for unweighted graph}
Given a weighted, but undirected graph $\mathcal{G} = <V,E> ,\{ (v_i, v_j, w_{(i,j)}) \in E, \forall i,j \in V )\}$, a vector $p^\alpha_s(u)$ to approximate the Personalized PageRank $\pi^\alpha_s(u)$ with dampling factor $\alpha$. We elided the constant $\alpha$ for clear notation.  

The recursive and linear definition of PPR tells us:
\begin{align}
    \overrightarrow {\pi}_{\alpha, s} &= \overrightarrow{v_s} \alpha  \sum_{i = 0}^{\infty}(1-\alpha)^{i} \bm P^{i} \\
            &= \overrightarrow{v_s} \alpha ( I  + \sum_{i = 1}^{\infty}(1-\alpha)^{i} \bm P^{i})\\
            &= \overrightarrow{v_s}  \alpha I  + \overrightarrow{v_s} \alpha \sum_{i = 1}^{\infty}(1-\alpha)^{i} \bm P^{i},\\
    R_\alpha &= \alpha  \sum_{i = 0}^{\infty}(1-\alpha)^{i} \bm P^{i} \\
            &= \alpha I + \alpha \sum_{i = 1}^{\infty}(1-\alpha)^{i} \bm P^{i} \\
            &= \alpha I + (1-\alpha) \bm P R_\alpha \\
    \overrightarrow {\pi}_{\alpha, s} &= \overrightarrow{v_s}  R_\alpha \\
            &=  \overrightarrow{v_s}  \alpha I  + \overrightarrow{v_s}  (1-\alpha) \bm P R_\alpha \\
            &=  \alpha \overrightarrow{v_s} + (1-\alpha)  \overrightarrow{v_s} \bm P R_\alpha \\
            &=  \alpha \overrightarrow{v_s} + (1-\alpha) \overrightarrow{\pi}_{(\alpha, v_s \bm P)},\\
            &=  \alpha \overrightarrow{v_s} + \overrightarrow{\pi}_{(\alpha, (1-\alpha) v_s \bm P)},\\            
\end{align}


Assign initial $v_s = \bm 1_s$, Eq.\ref{eq:ppv-reursion-recursive} gives the recursive formulation of PPR calculation. Starting from putting $\alpha v_s$ mass into $\pi(s)$, then propagation $(1-\alpha) v_s$ via the network ($ \bm P$) as the input $v_s$ for the next level nodes. The forward push algorithm essentially repeat the above process until there is no significant $v_s$ to be propagate.

The algorithm works for both un/directed or un/weighted graph, based on how to formulate $\bm P$. 


\begin{algorithm}[H]
\caption{$\textsc{ForwardPush}$ \cite{zhang2016approximate}}
\begin{algorithmic}[1]
\State \textbf{Input: }$\bm p_s, \bm r_s, \mathcal{G}, \epsilon, \beta = 0$
\While{$\exists u, r_s(u) > \epsilon d(u)$}
\State $\textsc{Push}(u)$
\EndWhile
\While{$\exists u, r_s(u) < -\epsilon d(u)$} 
\State $\textsc{Push}(u)$
\EndWhile
\State \Return $(\bm p_s, \bm r_s)$
\Procedure{Push}{$u$}
\State $p_s(u) \pluseq \alpha r_s(u)$
\For{$v \in \operatorname{Nei}(u)$}
\State $r_s(v) \pluseq (1-\alpha) r_s(u) (1-\beta) / d(u)$
\EndFor
\State $r_s(u) = (1-\alpha) r_s(u) \beta $
\EndProcedure
\end{algorithmic}
\label{algo:forward-local-push}
\end{algorithm}

\subsection{Dynamic PPR via Forward Push}
\label{appendix:dyn-ppr-push}
Similar to the formulation above, but we add an edge insertion or deletion.  Suppose at time $t+1$we insert an single new edge $(v_u, v_v, w_(u,v))$ to the graph $\bm G^{(t)}$, how to update the parameters?


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt   
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}[x=0.4pt,y=0.4pt,yscale=-1,xscale=1]
    %uncomment if require: \path (0,276); %set diagram left start at 0, and has height of 276
    
    
    %Shape: Circle [id:dp6177377526862062] 
    \draw   (246,98) .. controls (246,85.85) and (255.85,76) .. (268,76) .. controls (280.15,76) and (290,85.85) .. (290,98) .. controls (290,110.15) and (280.15,120) .. (268,120) .. controls (255.85,120) and (246,110.15) .. (246,98) -- cycle ;
    %Shape: Circle [id:dp1784403270352245] 
    \draw   (403,93) .. controls (403,80.85) and (412.85,71) .. (425,71) .. controls (437.15,71) and (447,80.85) .. (447,93) .. controls (447,105.15) and (437.15,115) .. (425,115) .. controls (412.85,115) and (403,105.15) .. (403,93) -- cycle ;
    %Shape: Circle [id:dp6416110255517944] 
    \draw   (347,216) .. controls (347,203.85) and (356.85,194) .. (369,194) .. controls (381.15,194) and (391,203.85) .. (391,216) .. controls (391,228.15) and (381.15,238) .. (369,238) .. controls (356.85,238) and (347,228.15) .. (347,216) -- cycle ;
    %Shape: Circle [id:dp3486444110500183] 
    \draw   (240,233) .. controls (240,220.85) and (249.85,211) .. (262,211) .. controls (274.15,211) and (284,220.85) .. (284,233) .. controls (284,245.15) and (274.15,255) .. (262,255) .. controls (249.85,255) and (240,245.15) .. (240,233) -- cycle ;
    %Shape: Circle [id:dp8249186864870216] 
    \draw   (100,177) .. controls (100,164.85) and (109.85,155) .. (122,155) .. controls (134.15,155) and (144,164.85) .. (144,177) .. controls (144,189.15) and (134.15,199) .. (122,199) .. controls (109.85,199) and (100,189.15) .. (100,177) -- cycle ;
    %Shape: Circle [id:dp9360878049566426] 
    \draw   (85,90) .. controls (85,77.85) and (94.85,68) .. (107,68) .. controls (119.15,68) and (129,77.85) .. (129,90) .. controls (129,102.15) and (119.15,112) .. (107,112) .. controls (94.85,112) and (85,102.15) .. (85,90) -- cycle ;
    %Shape: Circle [id:dp7730088104243199] 
    \draw   (174,32) .. controls (174,19.85) and (183.85,10) .. (196,10) .. controls (208.15,10) and (218,19.85) .. (218,32) .. controls (218,44.15) and (208.15,54) .. (196,54) .. controls (183.85,54) and (174,44.15) .. (174,32) -- cycle ;
    %Straight Lines [id:da933198006075885] 
    \draw    (129,90) -- (244,97.86) ;
    \draw [shift={(246,98)}, rotate = 183.91] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da896601842938809] 
    \draw    (141,167) -- (252.18,116.82) ;
    \draw [shift={(254,116)}, rotate = 155.71] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da20344875896867154] 
    \draw    (218,46) -- (253.53,78.65) ;
    \draw [shift={(255,80)}, rotate = 222.58] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da6413353007566629] 
    \draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=3.75]    (290,98) -- (396,98.95) ;
    \draw [shift={(402,99)}, rotate = 180.51] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=3.75]    (35.19,-10.59) .. controls (22.38,-4.5) and (10.65,-0.97) .. (0,0) .. controls (10.65,0.97) and (22.38,4.5) .. (35.19,10.59)   ;
    %Straight Lines [id:da16852402207129602] 
    \draw    (268,120) -- (262.13,209) ;
    \draw [shift={(262,211)}, rotate = 273.77] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da6238574957309465] 
    \draw    (287,111) -- (350.86,203.35) ;
    \draw [shift={(352,205)}, rotate = 235.34] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    
    % Text Node
    \draw (262,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {u};
    % Text Node
    \draw (418,84) node [anchor=north west][inner sep=0.75pt]   [align=left] {v};
    % Text Node
    \draw (257,224) node [anchor=north west][inner sep=0.75pt]   [align=left] {j};
    % Text Node
    \draw (363,211) node [anchor=north west][inner sep=0.75pt]   [align=left] {k};
    
    \end{tikzpicture}
    \caption{The new edge (u,v)}
    \label{fig:new-edge-example-appendix}
\end{figure}

The $p^t_s,r^t_s$ estimation has been converged to the true PPR. The addition of the edge may break the balance, specifically for :

\begin{align}
    p_s(u) + \alpha r_s(u) = (1-\alpha)\sum_{x \in N^{in}(u)}  \frac{p_s(x)}{d(x)}, \label{eq:u-invaraint} \\
    p_s(k) + \alpha r_s(k) = (1-\alpha)\sum_{x \in N^{in}(k)}  \frac{p_s(x)}{d(x)}, \\
    p_s(j) + \alpha r_s(j) = (1-\alpha)\sum_{x \in N^{in}(j)}  \frac{p_s(x)}{d(x)}, \\
    p_s(v) + \alpha r_s(v) = (1-\alpha)\sum_{x \in N^{in}(v)}  \frac{p_s(x)}{d(x)},
\end{align}


Where any equation evolve degree of node u break up (for node $j, k, v$). In order to fix the imbalance, we should adjust estimation $p_s, r_s$ at the expense of PPR value. 

We denote the updated degree is $d'(u)$ and $p'_s(u)$, for any node-u involved calculation, we want to make the value does not change, specifically :
\paragraph{Update $p_s(u)$}
\begin{align}
    \frac{p'_s(u)}{d'(u)} &= \frac{p_s(u)}{d(u)}, \\
    p'_s(u) &= d'(u) \frac{p_s(u)}{d(u)},\\
            &= (d(u)+1) \frac{p_s(u)}{d(u)},\\
            &= p_s(u) \frac{d(u)+1}{d(u)}, \label{eq:p-update}
\end{align}

Eq.\ref{eq:p-update} shows that we could scale $p_s(u)$ by a factor of $\frac{d(u)}{d(u)+1}$, but this adjustment for neighbors of node u further breaks up the invaraiant of node u itself in Eq. \ref{eq:u-invaraint}, thus we should adjust $r_s(u)$ to rebalance but increase the error of ppv.
\paragraph{Update $r_s(u)$}

\begin{align}
    p_s(u) + \alpha r_s(u) & = p_s'(u) + \alpha r_s'(u) = \sum_{x \in N^{in}(u)}  \frac{p_s(x)}{d(x)}, \\
    & = p_s(u)\frac{d(u)+1}{d(u)} + \alpha r_s'(u) ,\\
    & = p_s(u) + \frac{p_s(u)}{d(u)} + \alpha r_s'(u) ,  \\
    \Longrightarrow \alpha r_s'(u) - \alpha r_s(u) &= -\frac{p_s(u)}{d(u)},\\
    \alpha r_s'(u)  &= \alpha r_s(u) -\frac{p_s(u)}{d(u)},\\
    r_s'(u) &=  r_s(u) -\frac{p_s(u)}{\alpha d(u)},
\end{align}

\paragraph{Update $r_s(v)$}
\begin{align}
    p_s(v) + \alpha r_s(v) & = p_s(v) + \alpha (r_s(v)+\Delta) \\
    &= (1-\alpha) \left( \frac{p_s(u)}{d(u)} + \sum_{x \in N^{in}(v) \setminus \{ u \} }  \frac{p_s(x)}{d(x)} \right) \\
    \Longrightarrow \alpha \Delta &= (1-\alpha) \frac{p_s(u)}{d(u)}\\
    \Delta &= \frac{(1-\alpha)}{\alpha} \frac{p_s(u)}{d(u)}\\
    \Longrightarrow r_s'(v) &=  r_s(v) + \Delta \\
    &= r_s(v) + \frac{(1-\alpha)}{\alpha} \frac{p_s(u)}{d(u)}
\end{align}

\subsection{Extend unweighted Dynamic PPR to weighted graph}
\label{appendix:unweighted-ppr-update} %\label{appendix:dyn-ppr-push}

We extend the dynamic adjust to weighted graph.  In Figure \ref{fig:new-edge-example}, we add new edge $(u,v,w_{(u,v)})$ to the weighted-graph \footnote{weighted-graph: $D(u) = \sum_{i \in N(u)} w_{(u,i)}$}. Similar to the analysis of invariant properties for unweighted graph, we found that the insertion of edges breaks the balance of node $j,k,v$, since the node degree of $u$ is has been changed. To compensate the new edges (weights),  first, we adjust $p_s(u), r_s{u}$ to keep invariant of out-neighbors (node j,k).

Update of $p_s(u):$
\begin{align}
    \frac{p'_s(u)}{d'(u)} &= \frac{p_s(u)}{d(u)}, \\
    p'_s(u) &= d'(u) \frac{p_s(u)}{d(u)},\\
            &= (d(u)+w_{(u,v)}) \frac{p_s(u)}{d(u)},\\
            &= p_s(u) \frac{d(u)+w_{(u,v)}}{d(u)}, \label{eq:p-update-weighted}
\end{align}

Update of $r_s(u):$
\begin{align}
    p_s(u) + \alpha r_s(u) & = p_s'(u) + \alpha r_s'(u) = \sum_{x \in N^{in}(u)}  \frac{p_s(x)}{d(x)}, \\
    & = p_s(u)\frac{d(u)+w_{(u,v)}}{d(u)} + \alpha r_s'(u) ,\\
    & = p_s(u) + \frac{w_{(u,v)} p_s(u)}{d(u)} + \alpha r_s'(u) , \\
    \Longrightarrow \alpha r_s'(u) - \alpha r_s(u) &= -\frac{w_{(u,v)} p_s(u)}{d(u)},\\
    \alpha r_s'(u)  &= \alpha r_s(u) -\frac{w_{(u,v)} p_s(u)}{d(u)},\\
    r_s'(u) &=  r_s(u) -\frac{w_{(u,v)} p_s(u)}{\alpha d(u)} \label{eq:r-update-weighted}
\end{align}

\paragraph{Update $r_s(v)$}
\begin{align}
    p_s(v) + \alpha r_s(v) & = p_s(v) + \alpha (r_s(v)+\Delta) \\
    &= (1-\alpha) \left( \frac{w_{(u,v)} p_s(u)}{d(u)} + \sum_{x \in N^{in}(v) \setminus \{ u \} }  \frac{w_{(u,x)} p_s(x)}{d(x)} \right) \\
    \Longrightarrow \alpha \Delta &= (1-\alpha) \frac{ \Delta_{w_{(u,v)}} p_s(u)}{d(u)}\\
    \Delta &= \frac{(1-\alpha)}{\alpha} \frac{ \Delta_{w_{(u,v)}} p_s(u)}{d(u)}\\
    \Longrightarrow r_s'(v) &=  r_s(v) + \Delta \\
    &= r_s(v) + \frac{(1-\alpha)}{\alpha} \frac{\Delta_{w_{(u,v)}}p_s(u)}{d(u)}
\end{align}

\section{Linearity in PPR}
\begin{align}
   \pi_{\alpha, s}^{(k)} &= (1-\alpha) \pi_{\alpha, s}^{(k-1)} \bm P + \alpha v_s\\
  &= (1-\alpha)^{k} \pi_{\alpha, s}^{(0)} \bm P^{k} + \alpha \sum_{i = 1}^{k}(1-\alpha)^{i-1} v_s \bm P^{i-1} \\
%   &= \alpha \sum_{i = 0}^{k-1}(1-\alpha)^{i} \overrightarrow{v_s} \bm P^{i},  \\
  &= \alpha v_s \sum_{i = 0}^{k-1}(1-\alpha)^{i} \bm P^{i}, \text{assuming that }  \pi_{\alpha, s}^{(0)} = \bm 0 \\
  \text{Note that:  } when k \rightarrow \infty \\
  \pi_{\alpha, s} &= \alpha v_s \sum_{i = 0}^{k-1}(1-\alpha)^{i} \bm P^{i}\\
  &= v_s R_{\alpha}
\end{align}

It proves that $\pi_{\alpha, s} $ is the linear combination of $v_s$
}


% \red{it's hard for global pagerank to detect in this case} %EU-CORE-W1
% \red{it's easier to detect as degree increases more}  %EU-CORE-W3
% \red{netwalk is not aligned.}
% \red{DynAnom use node representation, AnomRank is considered as using one float number to represent the node.}

% Table \ref{tab:time-node-anomaly} present the running time of each algorithm for node-level anomaly localization. 
% NetWalk, as the node-level deep learning method, is not suitable for dynamic graphs of many snapshot since its complexity involves $T$. \red{to add more discussion}
% While AnomRank \red{todo}
\vspace{-2mm}
